C-PMI: Conditional Pointwise Mutual Information for Turn-level Dialogue Evaluation

Existing reference-free turn-level evaluation metrics for chatbots inadequately capture the interaction between the user and the system. Consequently, they often correlate poorly with human evaluations. To address this issue, we propose a novel model-agnostic approach that leverages Conditional Pointwise Mutual Information (C-PMI) to measure the turn-level interaction between the system and the user based on a given evaluation dimension. Experimental results on the widely used FED dialogue evaluation dataset demonstrate that our approach significantly improves the correlation with human judgment compared with existing evaluation systems. By replacing the negative log-likelihood-based scorer with our proposed C-PMI scorer, we achieve a relative 62.6% higher Spearman correlation on average for the FED evaluation metric. Our code is publicly available at https://github.com/renll/C-PMI.

==> 000todo.tex <==
%\section{Plan}
%\begin{itemize}

%\item Correlation with human rating
%\item Varying LLMs (GPT series and other Causal LMs)
%\item Ablation commonsense
%\item Exploring prompts
%\item Using DailyDialogue for surprise evaluation (Update this)
%\end{itemize}



%TODO  - (Please see below for specific todo)

%\begin{itemize}
    


%\item  ITIM METRIC  - Liliang TODO (algorithm and evaluating) - See FED for reference (April 14, 2023)

%\item Mankeerat TODO - dataset stats + baseline results for overall (April 14) 

%\item MEETING APRIL 14 (EVENING, Mankeerat, Liliang, Vicki and Revanth)

%\item Results and Conclusuion TODO (Mankeerat, Liliang, Vicki) (April 15)

%\item Add all citation and figures on overleaf todo (April 16)

%\item Read through by everyone + submitted to Prof Cheng (Monday April 17)

%\item  Mankeerat meeting with Heng + submit to heng for additional review (April - 18 - 19)

%\item (Vicki and Revanth TODO - overall setting up paper and fitting it to highlight novelty)

%\item https://doc2dial.github.io/workshop2023/

% \end{itemize}
